Compositional pre-processing for automated reasoning in dependent type theory

In the context of interactive theorem provers based on a dependent type theory, automation tactics (dedicated decision procedures, call of automated solvers, ...) are often limited to goals which are exactly in some expected logical fragment. This very often prevents users from applying these tactics in other contexts, even similar ones. This paper discusses the design and the implementation of pre-processing operations for automating formal proofs in the Coq proof assistant. It presents the implementation of a wide variety of predictible, atomic goal transformations, which can be composed in various ways to target different backends. A gallery of examples illustrates how it helps to expand significantly the power of automation engines.

==> defELPI.tex <==
\lstdefinelanguage{ELPI}{%
  basicstyle=\ttfamily\footnotesize\color{dkblue},
  morekeywords=[1]{pi},
  morekeywords=[2]{prod},
  morecomment=[l]\%,
  keywordstyle=[1]{\ttfamily\color{dkviolet}},
  keywordstyle=[2]{\ttfamily\color{dkgreen}},
  commentstyle={\ttfamily\color{gray}},
}%


==> defManSSR.tex <==
%=======================================================================
% Défini le style ssr Gallina pour les listings (Assia Mahboubi 2007)

\lstdefinelanguage{SSR} {

% Anything betweeen $ becomes LaTeX math mode
mathescape=true,
% Comments may or not include Latex commands
texcl=false,


% Vernacular commands
% here also come the novel commands presented in the paper
morekeywords=[1]{
Section, Class, End, Require, Import, Export,
Variable, Variables, Parameter, Parameters, Axiom, Hypothesis, Hypotheses,
Infix, Notation, Local, Tactic, Reserved, Scope, Open, Close, Bind, Delimit,
Definition, Let, Ltac, Fixpoint, CoFixpoint, Morphism, Relation,
Implicit, Arguments, Set, Unset, Contextual, Strict, Prenex, Implicits, Types,
Inductive, CoInductive, Record, Structure, Instance, Canonical, Coercion,
Theorem, Lemma, Corollary, Proposition, Fact, Remark, Example,
Proof, Goal, Save, Qed, Defined, Hint, Resolve, Rewrite, View,
Search, Show, Print, Printing, All, Graph, Projections, inside,
outside, Check, About, Fail, Abort,
Trakt, Add, Embedding, Symbol, Conversion},

% Gallina
morekeywords=[2]{forall, exists, exists2, fun, fix, cofix, struct,
      match, with, end, as, in, return, let, if, is, then, else,
      for, of, nosimpl},

% Sorts
morekeywords=[3]{Type, Prop},

% Various tactics, some are std Coq subsumed by ssr, for the manual purpose,
% here also come the novel tactics presented in the paper
morekeywords=[4]{
         pose, move, case, elim, apply, clear,
            hnf, intro, intros, generalize, rename, pattern, after,
	    destruct, induction, using, refine, inversion, injection,
         rewrite, congr, unlock, compute, vm_compute, native_compute,
            replace, fold, unfold, change, cutrewrite, simpl,
         have, suff, wlog, suffices, without, loss, nat_norm,
            assert, cut, trivial, revert, bool_congr, nat_congr, lia,
	 symmetry, transitivity, auto, split, left, right, autorewrite,
         snipe, scope, trakt, smt, hammer, congruence, sauto, scongruence, firstorder},

% Terminators
morekeywords=[5]{
         by, done, exact, reflexivity, tauto, romega, omega,
         assumption, solve, contradiction, discriminate, ring, field},


% Control
morekeywords=[6]{do, last, first, try, idtac, repeat},

% Various symbols
% For the ssr manual we turn off the prettyprint of formulas
% literate=
%	{->}{{$\rightarrow\,$}}2
% 	{->}{{\tt ->}}3
%	{<-}{{$\leftarrow\,$}}2
% 	{<-}{{\tt <-}}2
% 	{>->}{{$\mapsto$}}3
% 	{<=}{{$\leq$}}1
% 	{>=}{{$\geq$}}1
% 	{<>}{{$\neq$}}1
% 	{/\\}{{$\wedge$}}2
% 	{\\/}{{$\vee$}}2
% 	{<->}{{$\leftrightarrow\;$}}3
% 	{<=>}{{$\Leftrightarrow\;$}}3
% 	{:nat}{{$~\in\mathbb{N}$}}3
%	{fforall\ }{{$\forall_f\,$}}1
%	{forall\ }{{$\forall\,$}}1
%	{exists\ }{{$\exists\,$}}1
% 	{negb}{{$\neg$}}1
% 	{spp}{{:*:\,}}1
% 	{~}{{$\sim$}}1
% 	{\\in}{{$\in\;$}}1
% 	{/\\}{$\land\,$}1
% 	{:*:}{{$*$}}2
%	{=>}{{$\,\Rightarrow\ $}}1
% 	{=>}{{\tt =>}}2
% 	{:=}{{{\tt:=}\,\,}}2
% 	{==}{{$\equiv$}\,}2
% 	{!=}{{$\neq$}\,}2
% 	{^-1}{{$^{-1}$}}1
% 	{elt'}{elt'}1
%       {=}{{\tt=}\,\,}2
%       {+}{{\tt+}\,\,}2,

% Comments delimiters, we do turn this off for the manual
%comment=[s]{(*}{*)},

% Spaces are not displayed as a special character
showstringspaces=false,

% String delimiters
morestring=[b]",

% Size of tabulations
tabsize=2,

% Enables ASCII chars 128 to 255
extendedchars=true,

% Case sensitivity
sensitive=true,

% Automatic breaking of long lines
breaklines=true,

% Default style fors listings
basicstyle=\ttfamily\footnotesize,

% Position of captions is bottom
captionpos=b,

% Full flexible columns
columns=[l]spaceflexible,

% Style for (listings') identifiers
identifierstyle={\ttfamily\color{black}},
% Note : highlighting of Coq identifiers is done through a new
% delimiter definition through an lstset at the begining of the
% document. Don't know how to do better.

% Style for declaration keywords
keywordstyle=[1]{\ttfamily\color{dkviolet}},

% Style for gallina keywords
keywordstyle=[2]{\ttfamily\color{dkgreen}},

% Style for sorts keywords
keywordstyle=[3]{\ttfamily\color{lightblue}},

% Style for tactics keywords
keywordstyle=[4]{\ttfamily\color{dkblue}},

% Style for terminators keywords
keywordstyle=[5]{\ttfamily\color{red}},


%Style for iterators
%keywordstyle=[6]{\ttfamily\color{dkpink}},

% Style for strings
stringstyle=\ttfamily,

% Style for comments
%commentstyle=\rmfamily,

}

